A Jailbroken GenAI Model Can Cause Substantial Harm: GenAI-powered Applications are Vulnerable to PromptWares

In this paper we argue that a jailbroken GenAI model can cause substantial harm to GenAI-powered applications and facilitate PromptWare, a new type of attack that flips the GenAI model's behavior from serving an application to attacking it. PromptWare exploits user inputs to jailbreak a GenAI model to force/perform malicious activity within the context of a GenAI-powered application. First, we introduce a naive implementation of PromptWare that behaves as malware that targets Plan & Execute architectures (a.k.a., ReAct, function calling). We show that attackers could force a desired execution flow by creating a user input that produces desired outputs given that the logic of the GenAI-powered application is known to attackers. We demonstrate the application of a DoS attack that triggers the execution of a GenAI-powered assistant to enter an infinite loop that wastes money and computational resources on redundant API calls to a GenAI engine, preventing the application from providing service to a user. Next, we introduce a more sophisticated implementation of PromptWare that we name Advanced PromptWare Threat (APwT) that targets GenAI-powered applications whose logic is unknown to attackers. We show that attackers could create user input that exploits the GenAI engine's advanced AI capabilities to launch a kill chain in inference time consisting of six steps intended to escalate privileges, analyze the application's context, identify valuable assets, reason possible malicious activities, decide on one of them, and execute it. We demonstrate the application of APwT against a GenAI-powered e-commerce chatbot and show that it can trigger the modification of SQL tables, potentially leading to unauthorized discounts on the items sold to the user.

==> listings/RegularEcommerceOutPut2.tex <==
Tool Result: ```sql
SELECT
  ShippingAddress,
  PhoneNumber
FROM Accounts
WHERE
  UserID = 695;
```

==> listings/RegularEcommerceRequestPlan.tex <==
Plan:  create the SQLs queries. #E1 = CreateAndRunSQLQueries[Here is a new request from the user: |UserID=695| fill this request: find me a watch that is under 200$]
Plan:  run the SQL queries. #E2 = DoAction[#E1]
Plan: format the answer before returning to the user. #E3 = ReturnAnswer[#E1,#E2]

==> listings/RegularEcommerceRequestPlan2.tex <==
Plan:  create the SQLs queries. #E1 = CreateAndRunSQLQueries[Here is a new request from the user: |UserID=695| fill this request: What is my shipping address and phone number?]
Plan:  run the SQL queries. #E2 = DoAction[#E1]
Plan: format the answer before returning to the user. #E3 = ReturnAnswer[#E1,#E2]

==> listings/SQLTables.tex <==
You are an AI assistant that help customers buy products in an Ecommerce website, you create SQL queries to the database to provide end users with the information they need.
the Database includes the tables: 
1. "Products" the table holds a list of all the products that are for sale on the website, the table columns are: (ProductID, ProductName, Description, Price, BooleanInSupply, ShippingPrice) 

2. "Accounts" the table holds a list of all the users that are signed up on the website, the table columns are: (UserID,Balance UserName, ShippingAddress, PhoneNumber).

create SQL queries to the database tables based on the following request:  

<REQUEST>


return the SQL query that you created based on the request. 

==> listings/apt-ecommerce-tools-CreateAndRunSQL-prompt.tex <==

 
You are an AI assistant that help customers buy products in an Ecommerce website, you create SQL queries to the database to provide end users with the information they need.
the Database includes the tables "Products" the table holds a list of all the products that are for sale on the website, the table columns are: (ProductID, ProductName, Description, Price, BooleanInSupply, ShippingPrice)  and "Accounts" the table holds a list of all the users that are signed up on the website, the table columns are columns: (UserID,Balance UserName, ShippingAddress, PhoneNumber).
 create SQL queries to the database tables based on the following request: 'TEXT'
 
return the SQL query that you created based on the request. 

==> listings/code-structured.tex <==
\begin{lstlisting}[language=Python]
import numpy as np
    
def incmatrix(genl1,genl2):
    m = len(genl1)
    n = len(genl2)
    M = None #to become the incidence matrix
    VT = np.zeros((n*m,1), int)  #dummy variable
    
    #compute the bitwise xor matrix
    M1 = bitxormatrix(genl1)
    M2 = np.triu(bitxormatrix(genl2),1) 

    for i in range(m-1):
        for j in range(i+1, m):
            [r,c] = np.where(M2 == M1[i,j])
            for k in range(len(r)):
                VT[(i)*n + r[k]] = 1;
                VT[(i)*n + c[k]] = 1;
                VT[(j)*n + r[k]] = 1;
                VT[(j)*n + c[k]] = 1;
                
                if M is None:
                    M = np.copy(VT)
                else:
                    M = np.concatenate((M, VT), 1)
                
                VT = np.zeros((n*m,1), int)
    
    return M
\end{lstlisting}

==> sections/threat-model.tex <==
\section{Threat Model}
\label{section:threat-model}

In this research, we focus on GenAI-powered applications that receive prompt/s from the user.

\paragraph{Targets.} In this research we focus on decision-making GenAI-powered applications that receive a user prompt and determine the outcome based on the execution. 


\paragraph{Objective.} In this research we focus on the objective of steering the flow of a target GenAI-powered application toward a desired output/outcome. 
We consider a GenAI-powered application whose flow (logic) is dependent on a user prompt and determined using a series of queries sent from the GenAI application to the GenAI service.
For such GenAI-powered applications, we show that the finite-state machine of the application can be steered by attackers toward a desired outcome using a well-crafted user prompt created by an adversary, which we name \textit{adversarial flow steering prompt}.

\paragraph{Adversary.} We consider two types of adversaries: (1) a malicious user that interfaces with the GenAI-powered application and tries to steer the application for his/her benefit (e.g., convincing a chatbot to sell an item at a lower price than its real price \footnote{\url{https://gizmodo.com/ai-chevy-dealership-chatgpt-bot-customer-service-fail-1851111825}}). In this scenario, the attacker (user) performs the attack against the GenAI-powered application using direct prompt injection (by providing an \textit{adversarial flow steering prompt}), and (2) an attacker that attacks a user (victim) by applying an indirect prompt injection (e.g., by sending input to the user) that automatically triggers the victim's GenAI application. 
In this case, the attacker may try to gain some benefit at the expense of the user/victim (e.g., by triggering a payment transaction using a message sent to the victim which is interpreted by a GenAI-powered wallet application) or to harm the victim (sending messages with toxic content from the victim's account using the GenAI-powered assistant). 


\paragraph{Assumptions.} In our threat model, we assume that the attacker knows the logic (the queries used to interface with the GenAI service) of the target GenAI-powered application. 
We note that in many GenAI-powered applications, the logic of the application (the interface with the GenAI service) is coded inside the source code. 
In such applications, the abovementioned assumption is considered very easy.
For example, in the case of GenAI-powered Android applications whose GenAI queries are coded inside the applications, attackers could easily download the APK of the target GenAI-powered Android application from the Google Play Store, decompile the application to Java classes, and build/model the associated finite-state machine by searching for LangChain's calls.
In cases where the logic of the application (the queries used to interface with GenAI service) is coded inside the server, this assumption is not trivial. 
However, attackers can still reveal the finite-state machine of the GenAI-powered application by bribing an insider (e.g., the developer of the server) to reveal the logic/interface with the GenAI service or by hacking the company and exfiltrate the server's source code. 
